Large Language Models are Qualified Benchmark Builders: Rebuilding Pre-Training Datasets for Advancing Code Intelligence Tasks

Pre-trained code models rely heavily on high-quality pre-training data, particularly human-written reference comments that bridge code and natural language. However, these comments often become outdated as software evolves, degrading model performance. Large language models (LLMs) excel at generating high-quality code comments. We investigate whether replacing human-written comments with LLM-generated ones improves pre-training datasets. Since standard metrics cannot assess reference comment quality, we propose two novel reference-free evaluation tasks: code-comment inconsistency detection and semantic code search. Results show that LLM-generated comments are more semantically consistent with code than human-written ones, as confirmed by manual evaluation. Leveraging this finding, we rebuild the CodeSearchNet dataset with LLM-generated comments and re-pre-train CodeT5. Evaluations demonstrate that models trained on LLM-enhanced data outperform those using original human comments in code summarization, generation, and translation tasks. This work validates rebuilding pre-training datasets with LLMs to advance code intelligence, challenging the traditional reliance on human reference comments.

==> Tables/tab-eval-manual.tex <==
\begin{table}[]
\caption{The results of human evaluation.}
\label{tab:eval-manual}
\begin{tabular}{lccc}
\hline
\multicolumn{1}{l}{\multirow{2}{*}{Methods}} & Consistency & Conciseness & Completeness \\
\multicolumn{1}{c}{}                         & \multicolumn{3}{c}{Avg. (Std.)}          \\ \hline
Human References                             & 3.25 (0.95) & 3.83 (0.94) & 3.32 (0.98)  \\
StarCoder2-15B                               & 3.40 (0.84) & 3.81 (0.75) & 3.62 (0.84)  \\
Text-Davinci-003                             & 3.53 (0.94) & 3.75 (0.80) & 3.70 (0.95)  \\
CodeLlama-70B                                & 3.72 (0.80) & 3.78 (0.85) & 3.60 (0.88)  \\
DeepSeek-Coder-30B                           & 3.78 (0.70) & 3.70 (0.83) & 3.93 (0.70)  \\
GPT-3.5-turbo-0613                           & 3.92 (0.78) & 3.75 (0.84) & 3.95 (0.81)  \\
GPT-4-0613                                   & 4.04 (0.72) & 3.66 (0.88) & 4.12 (0.77)  \\ \hline
\end{tabular}
\end{table}

